List Decoding of Locally Repairable Codes

We show that locally repairable codes (LRCs) can be list decoded efficiently beyond the Johnson radius for a large range of parameters by utilizing the local error correction capabilities. The new decoding radius is derived and the asymptotic behavior is analyzed. We give a general list decoding algorithm for LRCs that achieves this radius along with an explicit realization for a class of LRCs based on Reed-Solomon codes (Tamo-Barg LRCs). Further, a probabilistic algorithm for unique decoding of low complexity is given and its success probability analyzed.

==> conclusion.tex <==
\section{Conclusion} \label{sec:conclusion}
In this work, we derived a new list decoding radius for locally repairable codes and gave an explicit algorithm that achieves it. The complexity and the list size are polynomial in the code length $n$ when considering scaling that preserves the number of local groups. The asymptotic behavior was analyzed and a simple probabilistic unique decoder was introduced. In future work, the decoding algorithm and list size should be studied more closely, as this work only includes a straightforward algorithm as a proof of work.
